SlimFlow: Training Smaller One-Step Diffusion Models with Rectified Flow

Diffusion models excel in high-quality generation but suffer from slow inference due to iterative sampling. While recent methods have successfully transformed diffusion models into one-step generators, they neglect model size reduction, limiting their applicability in compute-constrained scenarios. This paper aims to develop small, efficient one-step diffusion models based on the powerful rectified flow framework, by exploring joint compression of inference steps and model size. The rectified flow framework trains one-step generative models using two operations, reflow and distillation. Compared with the original framework, squeezing the model size brings two new challenges: (1) the initialization mismatch between large teachers and small students during reflow; (2) the underperformance of naive distillation on small student models. To overcome these issues, we propose Annealing Reflow and Flow-Guided Distillation, which together comprise our SlimFlow framework. With our novel framework, we train a one-step diffusion model with an FID of 5.02 and 15.7M parameters, outperforming the previous state-of-the-art one-step diffusion model (FID=6.47, 19.4M parameters) on CIFAR10. On ImageNet 64$\times$64 and FFHQ 64$\times$64, our method yields small one-step diffusion models that are comparable to larger models, showcasing the effectiveness of our method in creating compact, efficient one-step diffusion models.

==> 10822/text/cifar_table.tex <==
\begin{table*}[!t]
\centering
\footnotesize
\resizebox{0.95\linewidth}{!}{% <------ Don't forget this %
\begin{tabular}{l|l|cccc}
\toprule
Category & Method & \#Params \quad & NFE ($\downarrow$) \quad & FID ($\downarrow$) \quad & MACs ($\downarrow$) \\
\midrule 
\multirow{2}{*}{Teacher Model} & EDM \cite{karras2022elucidating} & 55.7M & 35 & 1.96 & 20.6G \\
& 1-Rectified Flow~\cite{liu2022flow} & 61.8M & 127 & 2.58 & 10.3G \\
\midrule 
\multirow{4}{*}{\shortstack[l]{{Diffusion}\\ {+ Pruning}}} 
& Proxy Pruning \cite{li2023not}
& 38.7M & 100 & 4.21 \\
& Diff-Pruning \cite{fang2024structural}
& 27.5M & 100 & 4.62 & 5.1G \\
& Diff-Pruning \cite{fang2024structural}
& 19.8M & 100 & 5.29 & 3.4G\\
& Diff-Pruning \cite{fang2024structural}
& 14.3M & 100 & 6.36 & 2.7G\\
\midrule 
\multirow{6}{*}{\shortstack[l]{{Diffusion}\\ {+ Fast Samplers}}} 
& AMED-Solver \cite{zhou2023fast} & 55.7M & 5 & 7.14 & 20.6G\\
& GENIE \cite{dockhorn2022genie}
& 61.8M & 10 & 5.28 & 10.3G\\
& 3-DEIS \cite{zhang2022fast}
& 61.8M & 10 & 4.17 & 10.3G\\
& DDIM \cite{song2020denoising}
& 35.7M & 10 & 13.36 & 6.1G\\
& DPM-Solver-2 \cite{lu2022dpm}
& 35.7M & 10 & 5.94 & 6.1G\\
& DPM-Solver-Fast \cite{lu2022dpm}
& 35.7M & 10 & 4.70 & 6.1G \\
% & DPM-solver++ \cite{lu2022dpm++} &  & 10 & 2.91 \\
% & AMED-Solver \cite{zhou2023fast} & 55.7M & 9 & \textbf{2.78} \\
\midrule 
\multirow{17}{*}{\shortstack[l]{{Diffusion}\\ {+ Distillation}}} 
& DSNO \cite{zheng2023fast}
& 65.8M & 1 & 3.78 & \\
& Progressive Distillation \cite{salimans2022progressive} & 60.0M & 1 & 9.12 & \\
& Score Mismatching~\cite{ye2023score}$^\dagger$ & 24.7M & 1 & 8.10 & \\
& TRACT \cite{berthelot2023tract} & 19.4M & 1 & 6.47 & \\
& Diff-Instruct~\cite{luo2023diff}$^\dagger$ & 55.7M & 1 & 4.53 & 20.6G \\
& TRACT \cite{berthelot2023tract} & 55.7M & 1 & 3.78 & 20.6G \\
& DMD \cite{yin2024one}$^\dagger$ & 55.7M & 1 & 3.77 & 20.6G \\
& Consistency Distillation (EDM teacher) \cite{song2023consistency} & 55.7M & 1 & {3.55}  & 20.6G \\
& 1-Rectified Flow (+distill) \cite{liu2022rectified}
 & 61.8M & 1 & 6.18 & 10.3G \\
& 2-Rectified Flow (+distill) \cite{liu2022rectified}
 & 61.8M & 1 & 4.85 & 10.3G\\
& 3-Rectified Flow (+distill) \cite{liu2022rectified}
 & 61.8M & 1 & 5.21 & 10.3G \\
& Consistency Distillation (EDM teacher) \cite{song2023consistency}$^*$ & 27.9M & 1 & 6.83 & 6.6G\\
& \textbf{\method{}} (EDM teacher) & 27.9M & 1 & 4.53 & 6.6G \\
& Knowledge Distillation~\cite{luhman2021knowledge}
 & 35.7M & 1 & 9.36 & 6.1G \\
& Consistency Distillation (EDM teacher) \cite{song2023consistency}$^*$ & 15.7M & 1 & 7.21 & 3.7G\\
% & Consistency Model (CD) \cite{song2023consistency} & 56.4M & 1 & \textbf{3.55}  \\
% & Consistency Model (CD) \cite{song2023consistency} (reproduced) & 15.9M & 1 & 7.91
%   \\
& \textbf{\method{}} (EDM teacher) & 15.7M & 1 & 5.02 & 3.7G \\
& \textbf{\method{}} (1-Rectified Flow teacher) & 15.7M & 1 & 5.81 & 3.7G  \\
\bottomrule
\end{tabular}}
\caption{
\label{table:cifar10}
Comparison on CIFAR10.
%$^\dagger$Methods that require adversarial-like training. 
`$*$' refers to reproduced results.
}
\end{table*}

==> 10822/text/experiment.tex <==
\section{Experiments}
\label{sec:expr}

In this section, we provide empirical evaluation of~\method{} and compare it with prior arts.
% \xc{don't use against, very aggresive}
The source code is available at \href{https://github.com/yuanzhi-zhu/SlimFlow}{https://github.com/yuanzhi-zhu/SlimFlow}. 
% \xc{code?}

% \begin{figure}[!t]
% \centering
% \begin{overpic}[width=0.99 \linewidth]{figures/one_step}% no need to specify the file extension
% \end{overpic}
% \caption{Random generated samples from our best one-step models on three different datasets. Left: CIFAR10 32$\times$32 (unconditional with 27.9M parameters); Mid: FFHQ 64$\times$64 (unconditional with 27.9M parameters); Right: ImageNet 64$\times$64 (conditional with 80.7M parameters).}
% \label{fig:one_step}
% \end{figure}


\subsection{Experimental Setup}
\label{sec:expr_setup}

\noindent\textbf{Datasets and Pre-trained Teacher Models.}~~
Our experiments are performed on the CIFAR10 \cite{krizhevsky2009learning} 32$\times$32 and the FFHQ \cite{karras2019style} 64$\times$64 datasets to demonstrate the effectiveness of \method{}. Additionally, we evaluated our method's performance on the ImageNet \cite{deng2009imagenet} 64$\times$64 dataset, focusing on conditional generation tasks.
% The pre-trained models we used to generate data pairs are from previous works Rectified Flow \cite{liu2022rectified} and EDM \cite{karras2022elucidating}.
The pre-trained large teacher models are adopted from the official checkpoints from previous works, Rectified Flow~\cite{liu2022rectified} and EDM~\cite{karras2022elucidating}.

\noindent\textbf{Implementation Details.}~~ For experiments on CIFAR10 32$\times$32 and the FFHQ 64$\times$64, we apply the U-Net architecture of NCSN$++$ proposed in \cite{song2020score}. For experiments on ImageNet 64$\times$64, we adopt a different U-Net architecture proposed in~\cite{dhariwal2021diffusion}.
% A more extensive exploration of architectural designs is reserved for future research.
% In our experiments involving both the CIFAR10 32$\times$32 and FFHQ 64$\times$64 datasets, we trained four distinct models with different sizes. 
% For the experiment on ImageNet 64$\times$64, we concentrated our testing on a single, smaller model size.
In the CIFAR10 experiments, we executed two sets of experiments with two different teacher models:
one is the pre-trained 1-Rectitied Flow~\cite{liu2022flow} and the other is the pre-trained EDM model~\cite{karras2022elucidating}. 
For all the other experiments, we adopt only the pre-trained EDM model as the large teacher model, unless specifically noted otherwise.
All the experiments are conducted on 4 NVIDIA 3090 GPUs.
In Distillation, we found replacing $v_\phi(\mathbf{x}_1, 1)$ with $v_{\phi'}(\mathbf{x}_1, 1)$ in~\cref{eq:2-step} leads to high empirical performance as $v_{\phi'}$ is a better one-step generator and speed up the training by saving one forward of the 2-rectified flow, so we keep that in our practice.
More details can be found in the Appendix.

\noindent\textbf{Evaluation Metrics.}~~
 We use the Fréchet inception distance (FID)\cite{heusel2017gans} to evaluate the quality of generated images. 
 In our experiments, we calculate the FID by comparing 50,000 generated images with the training dataset using Clean-FID \cite{parmar2022aliased}.
We also report the number of parameters (\#Params), Multiply-Add Accumulation (MACs), and FLoating-point OPerations per second (FLOPs) as metrics to compare the computational efficiency of different models.
It is important to note that in this paper, both MACs and FLOPs refer specifically to the computation required for a single forward inference pass through the deep neural network.
We use Number of Function Evaluations (NFEs) to denote the number of inference steps.

% \xc{please think about how to make readers excited before you write. what is the most exciting result you get? for readers of this paper, what do they care? do they care about straightness?}

\input{text/cifar_table}

\begin{figure}[!t]
\centering
\includegraphics[width=0.99 \linewidth]{figures/one_step}% no need to specify the file extension
\caption{Random generation from our best one-step small models on three different datasets. 
Left: CIFAR10 32$\times$32 (\#Params=27.9M). Mid: FFHQ 64$\times$64 (\#Params=27.9M). Right: ImageNet 64$\times$64 (\#Params=80.7M).}
\label{fig:one_step}
\end{figure}

\input{text/ffhq_imagenet_table}


\subsection{Empirical Results}
\noindent\textbf{\method{} on CIFAR10.}~~
% We report the results of \method{} on CIFAR10 in Table~\ref{table:cifar10}.
We report the results on CIFAR10 in Table~\ref{table:cifar10}.
For all the \method{} models, we train them using \anflow{} with the data pairs generated from the large teacher model for 800,000 iterations, then distilling them to one-step generator with flow-guided distillation for 400,000 iterations. 
For the consistency distillation baselines, we train them for 1,200,000 iterations with the same EDM teacher to ensure a fair comparison.
With only 27.9M parameters, one-step \method{} outperforms the 61.8M 2-Rectified Flow+Distill model (FID: $4.53 \leftrightarrow 4.85$). With the less than 20M parameters, \method{} gives better FID (5.02, \#Params=15.7M) than TRACT (6.48, \#Params=19.4M) and Consistency Distillation (7.21, \#Params=15.7M). Additional SlimFlow results with different parameters can be found in \cref{fig:fid_a} for comparison with Consistency Distillation \cite{song2023consistency} and in \cref{fig:fid_b} for comparison with 2-rectified flow.

\noindent\textbf{\method{} on FFHQ and ImageNet.}~~
We report the results of \method{} on FFHQ 64$\times$64 and ImageNet 64$\times$64 in Table~\ref{table:FFHQ_ImageNet}. For ImageNet 64$\times$64, the models are trained in the conditional generation scenarios where class labels are provided.
In FFHQ, our \method{} models surpasses BOOT with only 15.7M parameters. In ImageNet, \method{} obtains comparable performance as the 295.9M models trained with Consistency Training, BOOT and Progressive Distillation, using only 80.7M parameters. These results demonstrates the effectiveness of \method{} in training efficient one-step generative models.


\begin{figure}[!t]
\centering
\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{overpic}[width=0.9 \linewidth]{figures/fid_a}
\put(-3,60.){\color{black}{(a)}}
\end{overpic}
\phantomcaption
\label{fig:fid_a}
\end{subfigure}%
\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{overpic}[width=0.9 \linewidth]{figures/fid_b}
\put(-3.5,58.5){\color{black}{(b)}}
\end{overpic}
\phantomcaption
\label{fig:fid_b}
\end{subfigure}
\caption{
% (a) Final FID results of different model sizes on CIFAR10 in comparison with CD. (1flow) and (edm) represent data pairs from 1-flow \cite{liu2022rectified} and EDM model \cite{karras2022elucidating}. (b) Final FID results of different model sizes on the FFHQ dataset use EDM data pairs. \xc{change everything...}
(a) Comparison of models trained with different methods on CIFAR10. 
(b) Comparison between 2-rectified flow and the distilled one-step generator on CIFAR10.}
\label{fig:fid}
\end{figure}

\begin{figure}[!t]
\centering
\begin{overpic}[width=0.95 \linewidth]{figures/2flows_cifar.pdf}% no need to specify the file extension
% \put(76.5, 1.){\color{gray}{\line(0,1){41.4}}}
% \put(-1.5,34.3){\color{black}\scriptsize{EDM}}
\put(19,29.3){\color{black}\scriptsize{Multi-Step RK45}}
\put(67,29.3){\color{black}\scriptsize{One-Step Euler}}
\put(-1.5,25){\color{black}\scriptsize{27.9M}}
\put(-1.5,17.6){\color{black}\scriptsize{15.7M}}
\put(-1.5,10.5){\color{black}\scriptsize{7.0M}}
\put(-1.5,3.2){\color{black}\scriptsize{3.4M}}
\end{overpic}
% \includegraphics[width=0.95\textwidth]{figures/2flow_cifar.png}
\caption{CIFAR10 samples from 2-rectified flow models trained with \anflow{}. All images are generated with the same set of random noises. }
\label{fig:2flow_cifar}
\end{figure}

\noindent\textbf{Analysis of Annealing Reflow.}~~
We examine the straightening effect of \anflow{}.
We measured the straightness in the \anflow{} stage of models with different sizes on both the CIFAR10 32$\times$32 and the FFHQ 64$\times$64 dataset. 
Here, straightness is defined as in 
\cref{eq:straightness} following~\cite{liu2022flow, liu2023instaflow}.
% In \cref{fig:straightness_a}, there is a drastic reduction of straightness with the decrease of randomness $\beta$.
In \cref{fig:straightness_a}, straightness decreases as $\beta(k)$ gradually approaches 0.
In \cref{fig:straightness_b}, we observe that the straightness of the resulting 2-rectified flows decreases as their number of parameters increase.
In \cref{fig:2flow_cifar}, samples generated with four 2-rectified flows with different samplers are presented.
These results demonstrate the effectiveness of \anflow{} in learning straight generative flows.
%the final straightness of the 2-rectified flow is approximately inversely propositional to the number of parameters. 
% We choose the linear annealing schedule in all experiments, where $\beta=0$ after 300k training steps as indicated in \cref{fig:straightness_a}.
% In \cref{fig:heun_fid_a}, we tracked the FID along the \anflow{} on both CIFAR10 and FFHQ datasets and presented the FID results using Heun's sampler with an NFE of 3 alongside those from the RK45 sampler with a tolerance of 1e-3, yielding an NFE of approximately 50. 
% \begin{wraptable}{r}{0.4\textwidth}
%   \begin{center}
%   \setlength\tabcolsep{5pt}
%   \begin{tabular}{ccc}
%     \toprule
%     Annealing & H-Flip & FID \\
%     \midrule 
%      - & - & 5.84\\
%      - & \checkmark & 5.06\\
%     \checkmark & - & 5.46\\
%     \checkmark & \checkmark & 4.51\\
%     \bottomrule
%   \end{tabular}
%   \end{center}
% \caption{Ablation study on the reflow strategy of \method{}.}
% \label{tab:anneal_1}
% \end{wraptable} 
% We found that the results of Heun's sampler with NFE=3 are very close to that of RK45, which is consistent with the observations in \cref{fig:straightness_a}, underscores the straightness of the 2-flows.
% Additionally, \cref{fig:heun_fid_b} displays the FID curves at varying NFE levels using Heun's sampler.
% For all cases, we used the evenly discretized timesteps for simplicity.
% We found that Heun's sampler converges rapidly, producing FIDs close to those of RK45 even when NFE=3.
% Heun's sampler convergence very fast and can produce results remarkably close to those of RK45 with NFE=3. 
% This alignment with \cref{fig:straightness_a} further emphasizes the benefits of 2-rectified flows' straightness.
% In \cref{fig:2flow_cifar}, samples generated with four 2-rectified flows with different samplers are presented.



\begin{table*}[!t]
\centering
\footnotesize
\begin{minipage}{0.38\linewidth}
  \begin{center}
  \setlength\tabcolsep{5pt}
  \begin{tabular}{ccc}
    \toprule
    Annealing & H-Flip & FID ($\downarrow$) \\
    \midrule 
     - & - & 5.84\\
     - & \checkmark & 5.06\\
    \checkmark & - & 5.46\\
    \checkmark & \checkmark & 4.51\\
    \bottomrule
  \end{tabular}
  \end{center}
\caption{Ablation study on the reflow strategy of \method{}.}
\label{tab:anneal_1}
\end{minipage}
\hfill
\begin{minipage}{0.58\linewidth}
  \begin{center}
    \begin{tabular}{cc}
    \toprule
    $\beta(k)$ & FID ($\downarrow$) \\
    \midrule 
    $0$ & 5.06\\
    $\exp(-k / K_{step})$ & 4.78\\
    $\cos(\pi \min(1, k / 2K_{step})/2)$ & 4.79\\
    $(1+\cos(\pi \min(1,k/2K_{step})))/2$ & 4.70\\
    % $1 - \min(1, k / 2K_{step})$ & 4.73\\
    $1 - \min(1, k / 6 K_{step})$ & 4.51\\
    \bottomrule
    \end{tabular}
    \caption{
    \label{tab:anneal_2}
    Ablation study on the annealing strategy of \method{}. 
    Recall that $k$ is the number of training iterations. We set $K_{step}=50,000$.
    }
  \end{center}
\end{minipage}
\end{table*}


\subsection{Ablation Study}
\noindent\textbf{\anflow{}.}~~
We examine the design choices in \anflow{}. We train 2-rectified flow for 800,000 iterations and measure its FID with RK45 solver. 
% \begin{wraptable}{r}{0.6\textwidth}
%     \begin{center}
%     \begin{tabular}{cc}
%     \toprule
%     $\beta(k)$ & FID ($\downarrow$) \\
%     \midrule 
%     $0$ & 5.06\\
%     $\exp(-k / K_{step})$ & 4.78\\
%     $\cos(\pi \min(1, k / 2K_{step})/2)$ & 4.79\\
%     $(1+\cos(\pi \min(1,k/2K_{step})))/2$ & 4.70\\
%     % $1 - \min(1, k / 2K_{step})$ & 4.73\\
%     $1 - \min(1, k / 6 K_{step})$ & 4.51\\
%     \bottomrule
%     \end{tabular}
%     \caption{
%     \label{tab:anneal_2}
%     Ablation study on the annealing strategy of \method{}. 
%     Recall that $k$ is the number of training iterations. We set $K_{step}=50,000$.
%     }
%     \end{center}
% \end{wraptable}
In Table~\ref{tab:anneal_1}, we report the influence of the \anflow{} strategy and the effectiveness of exploiting the intrinsic symmetry of reflow. It can be observed that both the annealing strategy and the intrinsic symmetry improve the performance of 2-rectified flow, and their combination gives the best result. In Table~\ref{tab:anneal_2}, we analyze the schedule of $\beta(k)$. When $\beta(k)=0$, it is equivalent to training 2-rectified flow with random initialization. All other schedules output lower FID than $\beta(k)=0$, showing the usefulness of our annealing strategy. We adopt $\beta(k)=1-\min(1, k / 6 K_{step})$ as our default schedule in our experiments.

\noindent\textbf{Flow-Guided Distillation.}~~In Table~\ref{table:distillation}, we analyze the influence of different choices in our distillation stage. We found that using our 2-step regularization boosts the FID the the distilled one-step model. Using $\ell_2$ loss, it improves the FID from 7.90 to 7.30. Using LPIPS loss, it improves the FID from 6.43 to 5.81. 
We use the model architecture with 15.7M parameters for all ablation studies.


\begin{table*}[!t]
\centering
\setlength\tabcolsep{7pt}
\small{
\begin{tabular}{ccccc}
\toprule
Initialize from $v_\phi$ \qquad & Source of $\mathcal{D}_{distill}$ \qquad & Loss $\mathbb{D}$ \qquad & with $\mathcal{L}_{\text{2-step}}$ \qquad & FID \\ \midrule 
-        & 1-rectified flow $v_\theta$    & $\ell_2$  & -          & 12.09   \\ 
\checkmark        & 1-rectified flow $v_\theta$    & $\ell_2$    & -          & 8.98    \\
-        & 2-rectified flow $v_\phi$     & $\ell_2$   & -          & 9.19    \\ 
\checkmark        & 2-rectified flow $v_\phi$    & $\ell_2$   & -          & 7.90    \\ 
\checkmark        & 2-rectified flow $v_\phi$    & $\ell_2$    & \checkmark          & 7.30    \\
\checkmark        & 2-rectified flow $v_\phi$    & LPIPS        & -          & 6.43    \\
\checkmark        & 2-rectified flow $v_\phi$    & LPIPS        & \checkmark          & 5.81    \\ 
\bottomrule
\end{tabular}
}
\caption{Ablation study on the distillation stage of \method{} on CIFAR10. }
\label{table:distillation}
\end{table*}

\begin{figure}[!t]%[!t]
\centering
\begin{subfigure}[b]{0.48\textwidth}
\centering
\begin{overpic}[width=0.9 \linewidth]{figures/straightness_a}
\put(-3.5,60.){\color{black}{(a)}}
% \put(43.75,8.2){\color{gray}{\lines(0,1){55}}}
\end{overpic}
% \includegraphics[width=\textwidth]{figures/straightness_a.png}
% \caption{Left part of the figure}
\phantomcaption
\label{fig:straightness_a}
\end{subfigure}%
% Notice the comment sign (%) here to ensure no unwanted space is added
\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{overpic}[width=0.9 \linewidth]{figures/straightness_b}
\put(-3.5,57.5){\color{black}{(b)}}
\end{overpic}
% \includegraphics[width=\textwidth]{figures/straightness_b.png}
% \caption{Left part of the figure}
\phantomcaption
\label{fig:straightness_b}
\end{subfigure}
\caption{(a) Straightness of 2-rectified flows with different sizes during \anflow{}. (b) Final straightness of 2-rectified flows with different numbers of parameters. }
\label{fig:straightness}
\end{figure}


\iffalse
\begin{figure}[!t]%[!t]
\centering
\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{overpic}[width=0.9 \linewidth]{figures/heun_fid_a}
\put(-3,60.){\color{black}{(a)}}
\end{overpic}
\phantomcaption
\label{fig:heun_fid_a}
\end{subfigure}%
\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{overpic}[width=0.9 \linewidth]{figures/heun_fid_b}
\put(-3.5,58.5){\color{black}{(b)}}
\end{overpic}
\phantomcaption
\label{fig:heun_fid_b}
\end{subfigure}
\caption{(a) FID results of RK45 solver (NFEs $\approx$ 50 steps) and Heun solver (NFEs=3) during \anflow{}. (b) FID results of Heun solver with different NFEs on the last checkpoints. 
Measurements are on the models with 27.9M parameters using EDM data pairs.
% \xc{change everything...}
}
\label{fig:heun_fid}
\end{figure}
\fi

% \begin{table*}[!t]
% \centering
% \footnotesize
% \setlength\tabcolsep{5pt}
% \begin{minipage}{0.45\linewidth}
% % \begin{tabular}{cccc}
% % \toprule
% % \#Pairs &  Annealing & H-Flip & FID \\
% % \midrule 
% % 50000 & - & - & 5.84\\
% % 50000 & - & \checkmark & 5.06\\
% % 50000 & \checkmark & - & 5.46\\
% % 50000 & \checkmark & \checkmark & 4.51\\
% % %100000 & \checkmark & - & 4.48\\
% % % 100000 & \checkmark & \checkmark & 4.46\\
% % \bottomrule
% % \end{tabular}
% \begin{tabular}{ccc}
% \toprule
% Annealing & H-Flip & FID \\
% \midrule 
%  - & - & 5.84\\
%  - & \checkmark & 5.06\\
% \checkmark & - & 5.46\\
% \checkmark & \checkmark & 4.51\\
% \bottomrule
% \end{tabular}
% \caption{
% \label{table:2flow}
% Ablation study on the reflow strategy of \method{}. We measure the FID of 2-rectified flow with RK45 solver.
% \xc{training setting?}
% }
% \end{minipage}
% \hfill
% \begin{minipage}{0.5\linewidth}
% \begin{tabular}{cc}
% \toprule
% schedule of $\beta$ & FID ($\downarrow$) \\
% \midrule 
% $\exp(-k / K_{step})$ & 4.78\\
% $\cos(\pi \min(1, k / 2K_{step})/2)$ & 4.79\\
% $(1+\cos(\pi \min(1,k/2K_{step})))/2$ & 4.70\\
% $1 - \min(1, k / 2K_{step})$ & 4.73\\
% $1 - \min(1, k / 6 K_{step})$ & 4.51\\
% \bottomrule
% \end{tabular}
% \caption{
% \label{table:alpha_schedule}
% Ablation study on the annealing strategy of \method{}. We measure the FID of 2-rectified flow with RK45 solver.
% Recall that $k$ is the number of training iterations. Here, $K_{step}=50,000$.
% \xc{add $\beta(k)=0$}
% }
% \end{minipage}
% \end{table*}



==> 10822/text/ffhq_imagenet_table.tex <==

\begin{table*}[!t]
\centering
\footnotesize
\resizebox{0.95\linewidth}{!}{% <------ Don't forget this %
\begin{tabular}{l|l|ccccc}
\toprule
Dataset & Method & \#Params \quad & NFE ($\downarrow$) \quad & FID ($\downarrow$) \quad & MACs ($\downarrow$) \quad & FLOPs ($\downarrow$) \\ 
\midrule 
\multirow{5}{*}{\shortstack[l]{{FFHQ}\\ {64$\times$64}}}
% & FFHQ 64$\times$64 & & & & & \\ 
% \midrule 
& EDM \cite{karras2022elucidating} & 55.7M & 79 & 2.47 & 82.7G & 167.9G\\
& DDIM \cite{song2020denoising}
& 55.7M & 10 & 18.30 & 82.7G & 167.9G\\
& AMED-Solver \cite{zhou2023fast} & 55.7M & 5 & 12.54 & 82.7G & 167.9G \\
& BOOT \cite{gu2023boot} & 66.9M & 1 & 9.00 & 25.3G & 52.1G \\
& \textbf{\method{}} (EDM teacher) & 27.9M & 1 & 7.21 & 26.3G & 53.8G \\
& \textbf{\method{}} (EDM teacher) & 15.7M & 1 & 7.70 & 14.8G & 30.4G \\
\midrule
 % & & & & \\ 
\multirow{11}{*}{\shortstack[l]{{ImageNet}\\ {64$\times$64}}}
% ImageNet 64$\times$64 & & & & \\ 
& EDM \cite{karras2022elucidating} & 295.9M & 79 & 2.37 & 103.4G & 219.4G \\
& DDIM \cite{song2020denoising}
& 295.9M & 10 & 16.72 & 103.4G & 219.4G \\
& AMED-Solver \cite{zhou2023fast} & 295.9M & 5 & 13.75 & 103.4G & 219.4G \\
& DSNO \cite{zheng2023fast} & 329.2M & 1 & 7.83 &  \\
& Progressive Distillation \cite{salimans2022progressive} & 295.9M & 1 & 15.39 & 103.4G & 219.4G \\
& Diff-Instruct~\cite{luo2023diff} & 295.9M & 1 & 5.57 & 103.4G & 219.4G \\
& TRACT \cite{berthelot2023tract} & 295.9M & 1 & 7.43 & 103.4G & 219.4G \\
& DMD \cite{yin2024one} & 295.9M & 1 & 2.62 & 103.4G & 219.4G \\
& Consistency Distillation \cite{song2023consistency} & 295.9M & 1 & 6.20 & 103.4G & 219.4G \\
& Consistency Training \cite{song2023consistency} & 295.9M & 1 & 13.00 & 103.4G & 219.4G \\
& BOOT \cite{gu2023boot} & 226.5M & 1 & 16.30 & 78.2G & 157.4G \\
& \textbf{\method{}} (EDM teacher) & 80.7M & 1 & 12.34 & 31.0G & 67.8G \\
\bottomrule
\end{tabular}}
\caption{
\label{table:FFHQ_ImageNet}
Comparison on FFHQ 64$\times$64 and ImageNet 64$\times$64. 
% Baseline numbers are derived from Song et al.~\cite{song2023consistency}.
%$^\dagger$Methods that require adversarial-like training.
}
\end{table*}

==> 10822/text/method.tex <==
\section{\method{}}
\label{sec:method}

In this section, we introduce the \method{} framework for learning small, efficient one-step generative models.
% To effectively exploit the rectified flow framework in our setting, \method{} improves both reflow and distillation.
\method{} enhances the rectified flow framework by improving both the reflow and distillation stages.
For the reflow stage, we propose \anflow{}. This novel technique provides a warm-start initialization for the small student model. It smoothly transitions from training a 1-rectified flow to training a 2-rectified flow, accelerating the training convergence of the smaller network.
For the distillation stage, we propose Flow-Guided Distillation, which leverages the pre-trained 2-rectified flow as an additional regularization during distillation to improve the performance of the resulting one-step model.
%Combining both techniques yields \method{}, our framework for training efficient one-step diffusion model.
By combining these two techniques, \method{} creates a robust framework for training efficient one-step diffusion models that outperform existing methods in both model size and generation quality.

\subsection{\anflow{}}
\label{sec:an_flow}

The reflow procedure in the rectified flow framework trains a new, straighter flow $\mathbf{v}_\phi$ from the pre-trained 1-rectified flow $\mathbf{v}_\theta$, as described in ~\cref{eq:objective_reflow}. Typically, when $\mathbf{v}_\phi$ and $\mathbf{v}_\theta$ have the same model structure, $\mathbf{v}_\phi$ is initialized with $\mathbf{v}_\theta$'s weights to accelerate training. However, our goal of creating smaller models cannot adopt this approach, as $\mathbf{v}_\phi$ and $\mathbf{v}_\theta$ have different structures.
A naive solution would be to train a new 1-rectified flow using the smaller model with~\cref{eq:objective_rf} and use this as initialization. However, this strategy is time-consuming and delays the process of obtaining an efficient 2-rectified flow with the small model.

To address this challenge, we propose \anflow{}, which provides an effective initialization for the small student model without significantly increasing training time. This method starts the training process with random pairs, as in~\cref{eq:objective_rf}, then gradually shifts to pairs generated from the teacher flow, as in~\cref{eq:objective_reflow}.
%\xc{need fair comparison experiment}

Formally, given the teacher velocity field $\mathbf{v}_\theta$ defined by a large neural network $\theta$, the objective of \anflow{} is defined as,
\begin{equation}
\label{eq:objective_an_reflow}
\begin{aligned}
   \mathcal{L}^{k}_{\text{a-reflow}}(\phi):=&\mathbb{E}_{\mathbf{x}_1, \mathbf{x}'_1 \sim \pi_1} 
   \left[ \int_0^T \big \| \mathbf{v}_\phi (\mathbf{x}_t^{\beta(k)}, t ) - \left(\mathbf{x}_1^{\beta(k)} - \hat{\mathbf{x}}_0 \right ) \big \|_2^2 \mathrm{d}t \right], \\
   \text{where}~~~~& \mathbf{x}_t^{\beta(k)} = (1-t) \hat{\mathbf{x}}_0 + t \mathbf{x}_1^{\beta(k)}, \\ &\mathbf{x}_1^{\beta(k)} = \left ( \sqrt{1-\beta^2(k)} \mathbf{x}_1 + \beta(k) \mathbf{x}'_1  \right ), \\
   &\hat{\mathbf{x}}_0 = \mathrm{ODE}[\mathbf{v}_\theta](\mathbf{x}_1) = \mathbf{x}_1 + \int_1^0 \mathbf{v}_\theta(\mathbf{x}_{t},t) \mathrm{d} t.
\end{aligned}
\end{equation}
In~\cref{eq:objective_an_reflow}, $\mathbf{x}_1$ and $\mathbf{x}'_1$ are independent random samples from the initial distribution $\pi_1$. $k$ refers to the number of training iterations, and $\beta(k):\mathbb{N} \rightarrow [0,1]$ is a function that maps $k$ to a scalar between $0$ and $1$. The function $\beta(k)$ must satisfy two key conditions:
% \begin{enumerate}
%     \item $\beta(0)=1$: Substituting this condition into~\cref{eq:objective_an_reflow}, we see that $\mathcal{L}^{0}_{\text{a-reflow}}$ reduces to the rectified flow objective~\cref{eq:objective_rf} with a slight difference that $\hat{\mathbf{x}}_0$ is generated from the teacher model rather than sampled randomly from the training dataset $\pi_0$. Note that when $v_\theta$ is well-trained, $\hat{\mathbf{x}}_0$ also follows the target data distribution $\pi_0$.
%     \item $\beta(+\infty)=0$. Substituting this condition into~\cref{eq:objective_an_reflow},we see that $\mathcal{L}^{+\infty}_{\text{a-reflow}}$ reduces to the reflow objective~\cref{eq:objective_reflow}. Therefore, if we train our small student model with the \anflow{} objective long enough, it is equivalent to the original reflow procedure and guarantees to converge to a valid 2-rectified flow.
% \end{enumerate}
\begin{enumerate}
    \item $\beta(0)=1$: This initial condition reduces $\mathcal{L}^{0}_{\text{a-reflow}}$ to the rectified flow objective (\cref{eq:objective_rf}), with $\hat{\mathbf{x}}_0$ generated from the well-trained teacher model instead of being randomly sampled from $\pi_0$. Note that when $\mathbf{v}_\theta$ is well-trained, $\hat{\mathbf{x}}_0$ also follows the target data distribution $\pi_0$.
    \item $\beta(+\infty)=0$: This asymptotic condition ensures that $\mathcal{L}^{+\infty}_{\text{a-reflow}}$ converges to the reflow objective (\cref{eq:objective_reflow}), guaranteeing that the small model will eventually become a valid 2-rectified flow.
\end{enumerate}
% By choosing various schedule $\beta$, we transition from training the small student model with random pairs to the generated pairs from the teacher flow. This smooth transition provides the student model an appropriate initialization and directly outputs a small 2-rectified flow model.
By carefully choosing the schedule $\beta$, we create a smooth transition from training the small student model using random pairs to using pairs generated from the large teacher flow. This approach provides an appropriate initialization for the student model and directly outputs a small 2-rectified flow model, balancing efficiency and effectiveness in the training process.

\begin{figure}[!t]
\centering
\begin{overpic}[width=1.\linewidth]{figures/symmetry2}% no need to specify the file extension
% \put(76.5, 1.){\color{gray}{\line(0,1){41.4}}}
\put(1.5,32){\color{black}{(a)}}
\put(39.5,32){\color{black}{(b)}}
\put(78,32){\color{black}{(c)}}
\put(85,23){\color{black}\footnotesize{Original}}
\put(81,11){\color{black}\footnotesize{Horizontal Flip}}
\put(83,-1.){\color{black}\footnotesize{Vertical Flip}}
\end{overpic}
% \caption{(a) Samples generated with the model trained without any data augmentation. (b) Samples generated with a model trained with horizontal flip using the same initial noise. (c) Three image pairs generated with the model trained without any data augmentation using PF-ODE. From top to bottom: random noise and sample generated, horizontally flipped noise and corresponding sample, vertically flipped noise and corresponding sample.
% \xc{change to (c) only; add quantative curve}}
\caption{
(a) Generation from 1-Rectified Flow trained without data augmentation.
(b) Generation from the 1-Rectified Flow model in (a) after applying horizontal flip to the same set of random noises in (a). 
% \xc{change to follow this caption.}
(c) Horizontally flipping the noise results in horizontally flipped generated image, but vertical flip does not result in vertically flipped generated image.
}
\label{fig:symmetry}
\end{figure}

\noindent\textbf{Leveraging the Intrinsic Symmetry in Reflow Pairs.}~~
To perform reflow, a dataset of pair $(\mathbf{x}_1, \hat{\mathbf{x}}_0)$ is usually generated by the teacher flow before training the student model.
We find that the hidden symmetry in the pairs can be exploited to create new pairs without simulating the teacher flow.
Specifically, if the initial noise $\mathbf{x}_1$ is horizontally flipped (referred to as $\text{H-Flip}$), the corresponding image $\hat{\mathbf{x}}_0$ is also horizontally flipped.
As a result, for each generated pair $(\mathbf{x}_1, \hat{\mathbf{x}}_0)$, we can also add $\left( \text{H-Flip}(\mathbf{x}_1), \text{H-Flip}(\hat{\mathbf{x}}_0) \right )$ as a valid pair to double the sample size of our reflow dataset.

% While the coupling is robust no matter what kind of diffusion we use, we discover that there exists an intrinsic symmetry of diffusion (see \cref{fig:symmetry}).
% We initially observed that when two diffusion models are trained on an identical dataset—with one model utilizing horizontal flip data augmentation and the other not—the data samples generated from the same input noise are remarkably similar according to the PF-ODE.
% Furthermore, we show that for a model trained without any data augmentation, applying a horizontal flip to the initial noise results in a horizontally flipped generated image.
% This implies a data augmentation on the data pairs for the Rectifying that could potentially decrease the number of simulations of the teacher models.

\subsection{Flow-Guided Distillation}

Distillation is the other vital step in training one-step diffusion models with the rectified flow framework.
To distill the student flow, naive distillation~(\cref{eq:distill}) requires simulating the entire student 2-rectified flow with off-the-shelf solvers, e.g., Runge-Kutta 45 (RK45) solver, to get the distillation target $\mathrm{ODE}[\mathbf{v}](\mathbf{x}_1)$. 
In most times, practitioners generate a dataset of $M$ teacher samples in advance to training the student model, denoted as $\mathcal{D}_{distill} = \left\{\left(\mathbf{x}_1^{(i)}, \mathrm{ODE}[\mathbf{v}](\mathbf{x}_1^{(i)})\right)\right\}_{i=1}^M.$
Such simulation takes tens of steps,
leading to excessive time and storage for the distilled one-step model. 
On the one hand, for small models in our scenario, we want to use large $M$ to reach satisfying one-step models due to their limited capacity.
On the other hand, we also expect to avoid costly data generation in the distillation stage.

To balance this trade-off, we propose flow-guided distillation, where we complement the expensive direct distillation with an additional regularization. This regularization is based on few-step generation from the 2-rectified flow $\mathbf{v}_\phi$. When estimating the integration result of $\mathrm{ODE}[\mathbf{v}_\phi](\mathbf{x}_1)$, we can adopt the forward Euler solver,
\begin{equation}
    \mathbf{x}_{t_i} = \mathbf{x}_{t_{i+1}} + (t_{i} - t_{i+1}) \mathbf{v}_\phi(\mathbf{x}_{t_{i+1}}, t_{i+1}),~~~\forall i \in \{0, 1, \dots, N-1 \},
\end{equation}
where the $N$ time steps $\{t_i\}_{i=0}^N$ are defined by the user and $t_{0}=0, t_{N}=1$. 
To find an appropriate supervision for one-step simulation without cumbersome precise simulation with advanced solvers, a feasible choice is two-step simulation, which is,
\begin{equation}
\label{eq:euler_2_step}
\begin{aligned}
    \hat{\mathbf{x}}_0 = \mathbf{x}_1 - (1-t) \mathbf{v}_\phi(\mathbf{x}_1, 1) - t\mathbf{v}_\phi(\mathbf{x}_t, t).
\end{aligned}
\end{equation}
% \begin{equation}
% \begin{aligned}
%     \hat{\mathbf{x}}_0 =& \mathbf{x}_1 - \mathbf{v}_\phi(\mathbf{x}_t, t), \\
%    \text{where}~~~~& \mathbf{x}_t = \mathbf{x}_1 - (1-t) \mathbf{v}_\phi(\mathbf{x}_1, 1).
% \end{aligned}
% \end{equation}
Here, $t$ can be an intermediate time point between $(0, 1)$. Using this two-step approximation, we get another distillation loss,

\begin{equation}
\label{eq:2-step}
    \mathcal{L}_{\text{2-step}}(\phi'):= \mathbb{E}_{\mathbf{x}_1 \sim \pi_1} \left [ \int_0^1 \mathbb{D}(\mathbf{x}_1 - (1-t) \mathbf{v}_\phi(\mathbf{x}_1, 1) - t\mathbf{v}_\phi(\mathbf{x}_t, t), \mathbf{x}_1 - \mathbf{v}_{\phi'}(\mathbf{x}_1, 1)) \text{d} t \right].
\end{equation}
% \begin{equation}
% \label{eq:2-step}
%     \mathcal{L}_{\text{2-step}}(\phi'):= \mathbb{E}_{\mathbf{x}_1 \sim \pi_1} \left [ \int_0^1 \mathbb{D}(\mathbf{x}_1 - \mathbf{v}_\phi(\mathbf{x}_t, t), \mathbf{x}_1 - \mathbf{v}_{\phi'}(\mathbf{x}_1, 1)) \text{d} t \right].
% \end{equation}
While this two-step generation is not as accurate as the precise generation $\mathrm{ODE}[\mathbf{v}_\phi](\mathbf{x}_1)$ with Runge-Kutta solvers, it can serve as a powerful additional regularization in the distillation process to boost the performance of the student one-step model. Because two-step generation is fast, we can compute this term online as extra supervision to the student one-step model without the need to increase the size of $\mathcal{D}_{distill}$. Our final distillation loss is,
\begin{equation}
    \mathcal{L}_{\text{combined}}(\phi') = \mathcal{L}_{\text{distill}}(\phi') + \mathcal{L}_{\text{2-step}}(\phi').
\end{equation}
It is worth mentioning that we can use more simulation steps to improve the accuracy of the the few-step regularization within the computational budget. In our experiments, using two-step generation as our regularization already gives satisfying improvement. We leave the discovery of other efficient regularization as our future work. The whole procedure of our distillation stage is captured in Algorithm~\ref{alg:Distillation}.

\begin{algorithm}[t]
    \small
    \caption{Flow-Guided Distillation}
    \label{alg:Distillation}
    \begin{algorithmic}[1]
    \Require Pre-trained 2-rectified flow $v_\phi$, dataset $\mathcal{D}_{distill}$ generated with $v_\phi$.
    \State{Initialize the one-step student model $\mathbf{v}_{\phi'}$ with the weights of $\mathbf{v}_{\phi}$.}
    \Repeat
        \State{Randomly sample $\left(\mathbf{x}_1, \mathrm{ODE}[\mathbf{v}_\phi](\mathbf{x}_1) \right) \sim \mathcal{D}_{distill}$.}
        \State{Compute $\mathcal{L}_{\text{distill}}(\phi')$ with~\cref{eq:distill}.}

        \State{Randomly sample $\mathbf{x}_1 \sim \pi_1$.}
        \State{Compute $\mathcal{L}_{\text{2-step}}(\phi')$ with~\cref{eq:2-step}.}

        \State{Compute $\mathcal{L}_{\text{combined}}(\phi')=\mathcal{L}_{\text{distill}}(\phi')+\mathcal{L}_{\text{2-step}}(\phi')$.}
        \State{Optimize $\phi'$ with an gradient-based optimizer using $\nabla_{\phi'}\mathcal{L}_{\text{combined}}$.}

    \Until{$\mathcal{L}_{\text{combined}}$ converges.}
    
    \State{\textbf{Return} one-step model $v_{\phi'}$.}
    
    \end{algorithmic}
\end{algorithm}


==> 10822/text/related.tex <==
\section{Related Work}
\noindent\textbf{Reducing the Inference Steps of Diffusion Models.}~~ 
% Diffusion models generate new samples through a recurrent process, where a noisy image is iteratively fed into the neural network to be denoised.
% To accelerate them, various methods are proposed, and they can be categorized into two categories.
Diffusion models generate new samples through an iterative process, where a noisy image is repeatedly denoised by a neural network. To accelerate this process, researchers have proposed various methods, which can be categorized into two main approaches.

The first category is training-free methods, which aim to reduce the number of inference steps for existing diffusion models by optimizing the sampling process. By reformulating diffusion models into PF-ODEs \cite{song2020score}, numerous techniques are introduced to accelerate sampling while minimizing quality loss.
Some of the notable examples in this area include DDIM \cite{song2020denoising}, EDM \cite{karras2022elucidating}, DEIS \cite{zhang2022fast} and DPM-solver \cite{lu2022dpm}.
A recent advancement in this category is the AMED-Solver~\cite{zhou2023fast}, which leverages the mean value theorem to minimize discretization error, achieving high-quality generation with even fewer function evaluations.

Beyond these fast ODE salvers, distillation-based methods aim to achieve few-step sampling, or even one-step sampling, by training a new student model with the pre-trained multi-step diffusion models as teachers. 
Progressive Distillation~\cite{salimans2022progressive} proposed to repeatedly train a student network whose step size is twice as the step size of the teacher and set the student as a new teacher for the next round.
BOOT~\cite{gu2023boot} suggested distilling the knowledge of the teacher models in a data-free manner with the help of the signal-ODE.
Distribution Matching Distillation~\cite{yin2024one} extended the idea of Variational Score Distillation~\cite{wang2023prolificdreamer} to train a one-step generator by alternatively updating the one-step generator and a fake data score function.
Consistency models~\cite{song2023consistency, luo2023latent} are a new family of generative models that trains few-step diffusion models by applying consistency loss.
Additionally, several methods have incorporated adversarial training to enhance the performance of one-step diffusion models~\cite{ye2023score,kim2023consistency,xu2023ufogen}.

\noindent\textbf{Reducing the Size of Diffusion Models.}~~
% \xc{TODO: yuanzhi, write this part, add some citation} \xc{pruning, quantization, other structural modifications}
% The demand for low-budget or on-device applications often necessitates slim diffusion models, whereas the size of diffusion models such as Stable Diffusion is typically very large.
% To compress the size of pre-trained diffusion models, one can employ methods such as network pruning or Post-Training Quantization (PTQ) techniques.
The increasing demand for low-budget and on-device applications necessitates the development of compact diffusion models, as current state-of-the-art models like Stable Diffusion are typically very large. To address this challenge, researchers have explored various compression techniques, primarily focusing on network pruning and quantization methods.

% Network pruning involves trimming certain weights in the network and then fine-tuning the pruned model to maintain performance consistency with the pre-trained models. 
Network pruning involves selectively removing weights from the network and subsequently fine-tuning the pruned model to maintain performance comparable to the pre-trained version.
Diff-Pruning \cite{fang2024structural} utilizes Taylor expansion over pruned timesteps to identify non-contributory diffusion steps and important weights through informative gradients.
BK-SDM \cite{kim2023bk} discovers that block pruning combined with feature distillation is an efficient and sufficient strategy for obtaining lightweight models.

Another line of work is model quantization, 
which aims to reduce the storage and computational requirements of diffusion models during deployment \cite{wang2023towards, li2023q, he2023efficientdm, shang2023post, li2024q, huang2023tfmq}.
Q-diffusion \cite{li2023q} introduces timestep-aware calibration and split short-cut quantization, tailoring post-training quantization (PTQ) methods specifically for diffusion models.
%for tailored PTQ method for diffusion models.
EfficientDM \cite{he2023efficientdm} proposes a quantization-aware variant of the low-rank adapter (QALoRA), achieving Quantization-Aware Training (QAT)-level performance with PTQ-like efficiency.

% reusing information from previous steps \cite{ma2023deepcache,wimbauer2023cache}, and proposing better architecture design 

% In the future, we would explore more efficient small model architectures through pruning and adopt post-training techniques such as quantization to further improve efficiency.
%
% Since our method is orthogonal to post-training quantization and 

% Compared with prior works, \method{} considers the problem of simultaneously minimize the number of inference steps and the size of the neural network, targeting finding the most efficient diffusion models. 
In summary, \method{} advances the state of the art by addressing the dual challenge of minimizing both inference steps and neural network size, with the ultimate goal of developing the most efficient diffusion models.
While our approach shares some similarities with MobileDiffusion \cite{zhao2023mobilediffusion}, which also explores efficient structure design and acceleration of diffusion models, \method{} distinguishes itself in several key aspects:
% The work most related to ours is MobileDiffusion~\cite{zhao2023mobilediffusion}, which also discuss both efficient structure design and GAN-based acceleration of diffusion models. Some key differences are:
(1) \method{} is built upon the rectified flow framework, which provides more stable training dynamics than the GAN-based training used in MobileDiffusion; 
% (2) MobileDiffusion optimizes the network structure with fine-grained ablation study, but \method{} is a general framework that is applicable to any efficient networks and can thereby benefit from their efficient network.
(2) Unlike MobileDiffusion's focus on fine-grained specific network structure optimization, \method{} offers a general framework applicable to a wide range of efficient network architectures. This flexibility allows our approach to leverage advancements in efficient network design across the field, including MobileDiffusion's efficient text-to-image network.

==> text/experiment_old.tex <==
\section{Experiments}
\label{sec:expr}
% In this section, we provide empirical validation of the proposed \method{}, as detailed in \cref{sec:method}, and compare it against several prior studies. 
In this section, we provide empirical evaluation of~\method{} and compare it with prior arts.\xc{don't use against, very aggresive}
% Following the experimental setups described in \cref{sec:expr_setup}, we present the results for 2-flows trained using Annealing Rectifying and for the final distilled models in \cref{sec:result_2_flow} and \cref{sec:result_dis_flow}, respectively.
% Finally, we offer a comprehensive discussion of these findings to elucidate their significance and implications.
Source code will be released upon acceptance of the paper. \xc{code?}

\begin{figure}[!t]
\centering
\begin{overpic}[width=0.99 \linewidth]{figures/one_step}% no need to specify the file extension
\end{overpic}
\caption{Random generated samples from our best one-step models on three different datasets. Left: CIFAR10 32$\times$32 (unconditional with 27.9M parameters); Mid: FFHQ 64$\times$64 (unconditional with 27.9M parameters); Right: ImageNet 64$\times$64 (conditional with 80.7M parameters).}
\label{fig:one_step}
\end{figure}

% Besides, we apply our method to conditional image generation. 
% Furthermore, we extend the application of our method to encompass conditional image generation tasks.
% We demonstrate the utility and versatility of our method on unconditional generation
% by utilizing pairs from state-of-the-art flow and diffusion-based models.

\subsection{Experimental Setup}
\label{sec:expr_setup}

\noindent\textbf{Datasets and Pre-trained Teacher Models}~~
Our experiments are performed on the CIFAR10 \cite{krizhevsky2009learning} 32$\times$32 and the FFHQ \cite{karras2019style} 64$\times$64 datasets to demonstrate the effectiveness of \method{}. Additionally, we evaluated our method's performance on the ImageNet \cite{deng2009imagenet} 64$\times$64 dataset, focusing on conditional generation tasks.
% The pre-trained models we used to generate data pairs are from previous works Rectified Flow \cite{liu2022rectified} and EDM \cite{karras2022elucidating}.
The pre-trained large teacher models are adopted from the official checkpoints from previous works, Rectified Flow~\cite{liu2022rectified} and EDM~\cite{karras2022elucidating}.

\noindent\textbf{Implementation Details}~~ For experiments on CIFAR10 32$\times$32 and the FFHQ 64$\times$64, we apply the U-Net architecture of NCSN$++$ proposed in \cite{song2020score}. For experiments on ImageNet 64$\times$64, we adopt a different U-Net architecture proposed in~\cite{dhariwal2021diffusion}.
% A more extensive exploration of architectural designs is reserved for future research.
% In our experiments involving both the CIFAR10 32$\times$32 and FFHQ 64$\times$64 datasets, we trained four distinct models with different sizes. 
% For the experiment on ImageNet 64$\times$64, we concentrated our testing on a single, smaller model size.
In the CIFAR10 experiments, we executed two sets of experiments with two different teacher models:
one is the pre-trained 1-Rectitied Flow~\cite{liu2022flow} and the other is the pre-trained EDM model~\cite{karras2022elucidating}. 
For all the other experiments, we adopt only the pre-trained EDM model as the large teacher model, unless specifically noted otherwise.
All the experiments are conducted on 4 NVIDIA 3090 GPUs.
More details can be found in the Appendix.

\noindent\textbf{Evaluation Metrics}~~
 We use the Fréchet inception distance (FID)\cite{heusel2017gans} to evaluate the quality of generated images. 
 In our experiments, we calculate the FID by comparing 50,000 generated images with the training dataset using Clean-FID \cite{parmar2022aliased}.
We also report the number of parameters (\#Params), Multiply-Add Accumulation (MACs), and FLoating-point OPerations per second (FLOPs) as metrics to compare the computational efficiency of different models.

\xc{please think about how to make readers interested before you write. what is the most exciting result you get? for readers of this paper, what do they care? do they care about straightness?}

\subsection{Results of 2-Flows}
\label{sec:result_2_flow}
% We first validate that our approach can get straight 2-flows by Annealing Rectifying by examining their properties and generated samples.

\noindent\textbf{Straightness.}
We first measured the straightness defined in \cref{eq:straightness} in the Annealing Rectifying phase on four models with different sizes on both the CIFAR10 32$\times$32 dataset and the FFHQ 64$\times$64 dataset. As illustrated in \cref{fig:straightness_a}, there is a drastic decrease of straightness with the decrease of randomness $\beta$.
In \cref{fig:straightness_b}, we found that the final straightness of the 2-flows is approximately inversely propositional to the number of parameters in the models. We choose the linear annealing schedule in all experiments, where $\beta=0$ after 300k training steps as indicated in \cref{fig:straightness_a}.

\begin{figure}[!t]%[!t]
\centering
\begin{subfigure}[b]{0.48\textwidth}
\centering
\begin{overpic}[width=0.9 \linewidth]{figures/straightness_a}
\put(-3.5,60.){\color{black}{(a)}}
\put(43.75,8.2){\color{gray}{\line(0,1){55}}}
\end{overpic}
% \includegraphics[width=\textwidth]{figures/straightness_a.png}
% \caption{Left part of the figure}
\phantomcaption
\label{fig:straightness_a}
\end{subfigure}%
% Notice the comment sign (%) here to ensure no unwanted space is added
\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{overpic}[width=0.9 \linewidth]{figures/straightness_b}
\put(-3.5,57.5){\color{black}{(b)}}
\end{overpic}
% \includegraphics[width=\textwidth]{figures/straightness_b.png}
% \caption{Left part of the figure}
\phantomcaption
\label{fig:straightness_b}
\end{subfigure}
\caption{(a) Straightness of 2-flow models with different sizes during Annealing Rectifying. (b) Final straightness of 2-flow models with different numbers of parameters. Straightness is calculated using 100 Euler steps and averaging over 256 images.}
\label{fig:straightness}
\end{figure}


\begin{figure}[!t]%[!t]
\centering
\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{overpic}[width=0.9 \linewidth]{figures/heun_fid_a}
\put(-3,60.){\color{black}{(a)}}
\end{overpic}
\phantomcaption
\label{fig:heun_fid_a}
\end{subfigure}%
\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{overpic}[width=0.9 \linewidth]{figures/heun_fid_b}
\put(-3.5,58.5){\color{black}{(b)}}
\end{overpic}
\phantomcaption
\label{fig:heun_fid_b}
\end{subfigure}
\caption{(a) FID results of RK45 solver (NFE $\approx$ 50 steps) and Heun solver (NFE=3) during Annealing Rectifying. \xc{change legend} (b) FID results of Heun solver with different NFE on the last checkpoint. Measurements are on the models with 27.9M parameters using EDM data pairs.}
\label{fig:heun_fid}
\end{figure}



\begin{figure}[!t]
\centering
\begin{overpic}[width=0.95 \linewidth]{figures/2flows_cifar}% no need to specify the file extension
% \put(76.5, 1.){\color{gray}{\line(0,1){41.4}}}
\put(-1.5,34.3){\color{black}\scriptsize{EDM}}
\put(19,29.3){\color{black}\scriptsize{RK45: NFE $\approx$ 50}}
\put(67,29.3){\color{black}\scriptsize{Euler: one-step}}
\put(-1.5,25){\color{black}\scriptsize{27.9M}}
\put(-1.5,17.6){\color{black}\scriptsize{15.7M}}
\put(-1.5,10.5){\color{black}\scriptsize{7.0M}}
\put(-1.5,3.2){\color{black}\scriptsize{3.4M}}
\end{overpic}
\caption{CIFAR10 samples from 2-flow models with different model sizes and samplers. The result from EDM with Heun's sampler (NFE=18) is in the upper part for reference. All images are generated with the same random noise.}
\label{fig:2flow_cifar}
\end{figure}

\noindent\textbf{Performance.}
In \cref{fig:heun_fid_a}, we tracked the FID along the Annealing Rectifying of the largest models, which have 27.9 million parameters, on both CIFAR10 and FFHQ datasets.
We present the FID results using Heun's sampler with an NFE of 3, alongside those from the RK45 sampler with a tolerance of 1e-3, yielding an NFE of approximately 50. 
% We found that the results of Heun's sampler with NFE=3 are very close to that of RK45, which is consistent with the observations in \cref{fig:straightness_a}, underscores the straightness of the 2-flows.
Additionally, \cref{fig:heun_fid_b} displays the FID curves at varying NFE levels using Heun's sampler.
For all Heun's samplers, we used the evenly discretized timesteps for simplicity.
We found that Heun's sampler converges rapidly, producing FIDs close to those of RK45 even when NFE=3.
% Heun's sampler convergence very fast and can produce results remarkably close to those of RK45 with NFE=3. 
This alignment with \cref{fig:straightness_a} further emphasizes the benefits of 2-flows' straightness.
In \cref{fig:2flow_cifar}, samples generated with four 2-flows with different samplers are presented.


\begin{table*}[!t]
\centering
\footnotesize
\begin{minipage}{0.45\linewidth}
\begin{tabular}{cccc}
\toprule
\#pairs\quad & \quad annealing\quad & \quad H-Flip\quad & \quad FID ($\downarrow$) \\
\midrule 
50000 & - & - & 5.84\\
50000 & - & \checkmark & 5.06\\
50000 & \checkmark & - & 5.46\\
50000 & \checkmark & \checkmark & 4.51\\
100000 & \checkmark & - & 4.48\\
% 100000 & \checkmark & \checkmark & 4.46\\
\bottomrule
\end{tabular}
\caption{
\label{table:2flow}
FID of 2-flows with RK45 sampler.
}
\end{minipage}
\hfill
\begin{minipage}{0.5\linewidth}
\begin{tabular}{cc}
\toprule
schedule of $\beta$ & FID ($\downarrow$) \\
\midrule 
$\exp(-\text{step} / 50000)$ & 4.78\\
$\cos(\pi/2 * \min(1, \text{step}/100000))$ & 4.79\\
$(1+\cos(\pi*\min(1,\text{step}/100000)))/2$ & 4.70\\
$1 - \min(1, \text{step} / 100000)$ & 4.73\\
$1 - \min(1, \text{step} / 300000)$ & 4.51\\
\bottomrule
\end{tabular}
\caption{
\label{table:alpha_schedule}
FID of 2-flows using different annealing schedules with RK45 sampler.
}
\end{minipage}
\end{table*}

\noindent\textbf{Ablation on The Annealing and Data Augmentation.}
We did ablation studies to reveal the importance of the proposed method. In this experiment, we use the CIFAR10 data pairs from 1-flow in \cite{liu2022rectified} and a model size of 15.7M parameters. As illustrated in \cref{table:2flow}, with both an annealing schedule and horizontal flip (H-flip) applied, the 2-flow model achieves the lowest FID on CIFAR10 of 4.51 with data pairs from 1-flow. And the horizontal flip data augmentation can help reduce the required data pairs. 
Notably when a 1-flow of size 15.7M is available, we can initialize from it instead of using the Annealing Rectifying technique and achieve an even better FID of 4.34 with H-Flip, but this is usually not feasible.
We also ablated on the schedule of randomness $\beta$ in \cref{table:alpha_schedule} and found out a linear schedule works best in practice.


\subsection{Results of Distilled Flows}
\label{sec:result_dis_flow}


\noindent\textbf{Effect of the New Loss.} In \cref{table:distillation}, we did a series of experiments on the CIFAR10 dataset to show that the additional loss can help improve the distillation (the last four rows). 
The data pairs are generated by 1-flow in \cite{liu2022rectified} and the number of parameters is 15.7M. 
We found that LPIPS loss with the additional loss resulted in the best distilled model.
To demonstrate the effect of the new loss, we also made experiments on the original 2-flow checkpoint. Compared to the distillation checkpoint provided in the Rectified Flows, the new distilled model gains an improvement of 0.3 in FID. 


% \begin{table*}[!t]
% \centering
% \footnotesize
% \begin{minipage}{0.4\linewidth}
% \begin{tabular}{ccc}
% \toprule
% $d(\cdot,\cdot)$\quad & \quad use 2-flow \quad & \quad FID ($\downarrow$) \\
% \midrule 
% $l_2$ & - & 7.90\\
% $l_2$ & \checkmark & 7.30\\
% LPIPS & - & 6.43\\
% LPIPS & \checkmark & 5.81\\
% \bottomrule
% \end{tabular}
% \caption{
% \label{table:distillation}
% FID of distilled flows using different loss-type $d(·, ·)$ and with or without 2-flow regularization loss. 
% }
% \end{minipage}
% \hfill
% \begin{minipage}{0.58\linewidth}
% \begin{tabular}{ccccc}
% \toprule
% finetune \qquad & data pairs \qquad & $d(\cdot,\cdot)$ \qquad & use 2-flow \qquad & FID ($\downarrow$) \\
% \midrule 
% \checkmark & 2-flow & $l_2$ & - & 7.90 \\
% - & 2-flow & $l_2$ & - & 9.19 \\
% \checkmark & 1-flow & $l_2$ & - & 8.98 \\
% - & 1-flow & $l_2$ & - & 12.09 \\
% \bottomrule
% \end{tabular}
% \caption{
% \label{table:distillation_2}
% FID of distilled flows.
% }
% \end{minipage}
% \end{table*}

\begin{table*}[!t]
\centering
\begin{tabular}{ccccc}
\toprule
finetune initial \qquad & source of data pairs \qquad & loss $d(\cdot,\cdot)$ \qquad & Flow-Guided Distillation \qquad & FID ($\downarrow$) \\ \midrule 
-        & 1-flow     & $l_2$  & -          & 12.09   \\ 
\checkmark        & 1-flow     & $l_2$    & -          & 8.98    \\
-        & 2-flow     & $l_2$   & -          & 9.19    \\ 
\checkmark        & 2-flow     & $l_2$   & -          & 7.90    \\ 
\checkmark        & 2-flow     & $l_2$    & \checkmark          & 7.30    \\
\checkmark        & 2-flow     & LPIPS        & -          & 6.43    \\
\checkmark        & 2-flow     & LPIPS        & \checkmark          & 5.81    \\ 
\bottomrule
\end{tabular}
\caption{Ablation study on the distillation stage of \method{} on CIFAR10. We use the model with 15.7M parameters. \xc{change the first row to multirow}}
\label{table:distillation}
\end{table*}


\noindent\textbf{Toggle the Distillation.}
In previous works \cite{liu2022rectified, liu2023instaflow}, researchers found that improving transport costs significantly facilitates the distillation process. 
We further validate this point in \cref{table:distillation} by delving deeper into the significance of model initialization and the origin of data pairs for distillation. 
% The experimental setting is the same as in \cref{table:distillation}.
The choices for model initialization include finetuning from 2-flows or initializing randomly, while the data pairs can originate from either 1-flow or 2-flow models.
Our findings indicate that starting with a randomly initialized model and employing data pairs from 1-flow will lead to inferior performance of the final one-step models.
This suggests that it is essential to make the ODE trajectory sufficiently regular and smooth before applying distillation.

\noindent\textbf{One-step Performance.} The final results on the CIFAR10 dataset is exhibited in \cref{fig:fid_a} and \cref{table:cifar10}. We reproduced CD for all four architectures and comparing with our results using 1-flow data and EDM data. The teacher models are the same for fair comparison. We found our method beat consistency models in distillation by a large margin under the same model sizes.
The results on the FFHQ dataset can be found in \cref{fig:fid_b} and \cref{table:FFHQ_ImageNet}. 
% \noindent\textbf{Results on ImageNet 64$\times$64.}
Due to the limit of computational resources, we only tried one small model on the ImageNet 64$\times$64 dataset. With a total of 80.7M parameters and MACs of 31.0G (less than one-third of the teacher model), the 2-flow model achieved an FID of 8.89 with RK45 sampler and the final one-step model achieved an FID of 12.34 (see \cref{table:FFHQ_ImageNet}). 
\cref{fig:one_step} shows some non-cherry-picked samples generated by the one-step distilled flows. In conclusion, our \method{} can achieve competitive distillation performance on small models.

\begin{table*}[!t]
\centering
\footnotesize
\resizebox{0.88\linewidth}{!}{% <------ Don't forget this %
\begin{tabular}{llcccc}
\toprule
Category & Method & \#Params \quad & NFE ($\downarrow$) \quad & FID ($\downarrow$) \quad & MACs ($\downarrow$) \\
\midrule 
Teacher & EDM \cite{karras2022elucidating} & 55.7M & 35 & 1.96 & 20.6G \\
\midrule 
\multirow{4}{*}{\shortstack[l]{{Diffusion}\\ {+ Pruning}}} 
& Diff-Pruning \cite{fang2024structural}
& 14.3M & 100 & 6.36 & 2.7G\\
& Diff-Pruning \cite{fang2024structural}
& 19.8M & 100 & 5.29 & 3.4G\\
& Diff-Pruning \cite{fang2024structural}
& 27.5M & 100 & 4.62 & 5.1G \\
& Proxy Pruning \cite{li2023not}
& 38.7M & 100 & 4.21 \\
\midrule 
\multirow{6}{*}{\shortstack[l]{{Diffusion}\\ {+ Samplers}}} & DDIM \cite{song2020denoising}
& 35.7M & 10 & 13.36 & 6.1G\\
& DPM-solver-2 \cite{lu2022dpm}
& 35.7M & 10 & 5.94 & 6.1G\\
& DPM-solver-fast \cite{lu2022dpm}
& 35.7M & 10 & 4.70 & 6.1G \\
& GENIE (learned sampler) \cite{dockhorn2022genie}
& 61.8M & 10 & 5.28 & 10.3G\\
& 3-DEIS \cite{zhang2022fast}
& 61.8M & 10 & 4.17 & 10.3G\\
% & DPM-solver++ \cite{lu2022dpm++} &  & 10 & 2.91 \\
& AMED-Solver \cite{zhou2023fast} & 55.7M & 5 & 7.14 & 20.6G\\
% & AMED-Solver \cite{zhou2023fast} & 55.7M & 9 & \textbf{2.78} \\
\midrule 
\multirow{17}{*}{\shortstack[l]{{Diffusion}\\ {+ Distillation}}} & Knowledge Distillation~\cite{luhman2021knowledge}
 & 35.7M & 1 & 9.36 & 6.1G \\
& DSNO \cite{zheng2023fast}
& 65.8M & 1 & 3.78 \\
& 1-Rectified Flow (+distill) \cite{liu2022rectified}
 & 61.8M & 1 & 6.18 & 10.3G \\
& 2-Rectified Flow (+distill) \cite{liu2022rectified}
 & 61.8M & 1 & 4.85 & 10.3G\\
& 3-Rectified Flow (+distill) \cite{liu2022rectified}
 & 61.8M & 1 & 5.21 & 10.3G \\
& Progressive Distillation \cite{salimans2022progressive} & 60.0M & 1 & 9.12 \\
& Diff-Instruct~\cite{luo2023diff}$^\dagger$ & 55.7M & 1 & 4.53 & 20.6G \\
& Score Mismatching~\cite{ye2023score}$^\dagger$ & 24.7M & 1 & 8.10 \\
& TRACT \cite{berthelot2023tract} & 55.7M & 1 & 3.78 & 20.6G \\
& TRACT \cite{berthelot2023tract} & 19.4M & 1 & 6.47 \\
& DMD \cite{yin2024one}$^\dagger$ & 55.7M & 1 & 3.77 & 20.6G \\
& Consistency Model (CD, EDM) \cite{song2023consistency} & 55.7M & 1 & {3.55}  & 20.6G \\
& Consistency Model (CD) \cite{song2023consistency}$^*$ & 27.9M & 1 & 6.83 & 6.6G\\
& Consistency Model (CD) \cite{song2023consistency}$^*$ & 15.7M & 1 & 7.21 & 3.7G\\
% & Consistency Model (CD) \cite{song2023consistency} & 56.4M & 1 & \textbf{3.55}  \\
% & Consistency Model (CD) \cite{song2023consistency} (reproduced) & 15.9M & 1 & 7.91
%   \\
& \textbf{\method{}} (EDM data) & 27.9M & 1 & 4.53 & 6.6G \\
& \textbf{\method{}} (EDM data) & 15.7M & 1 & 5.02 & 3.7G \\
& \textbf{\method{}} (1-flow data) & 15.7M & 1 & 5.81 & 3.7G  \\
\bottomrule
\end{tabular}}
\caption{
\label{table:cifar10}
Sample quality and model efficiency comparison on CIFAR-10. Baseline numbers are derived from Song \etal ~\cite{song2023consistency}. $^\dagger$Methods that require adversarial-like training. $^*$Reproduced results.
\xc{Do CD and SlimFlow use the same number of training steps?}
}
\end{table*}



\begin{figure}[!t]
\centering
\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{overpic}[width=0.9 \linewidth]{figures/fid_a}
\put(-3,60.){\color{black}{(a)}}
\end{overpic}
\phantomcaption
\label{fig:fid_a}
\end{subfigure}%
\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{overpic}[width=0.9 \linewidth]{figures/fid_b}
\put(-3.5,58.5){\color{black}{(b)}}
\end{overpic}
\phantomcaption
\label{fig:fid_b}
\end{subfigure}
\caption{(a) Final FID results of different model sizes on CIFAR10 in comparison with CD. (1flow) and (edm) represent data pairs from 1-flow \cite{liu2022rectified} and EDM model \cite{karras2022elucidating}. (b) Final FID results of different model sizes on the FFHQ dataset use EDM data pairs.}
\label{fig:fid}
\end{figure}



\begin{table*}[ht]
\centering
\footnotesize
\resizebox{0.9\linewidth}{!}{% <------ Don't forget this %
\begin{tabular}{llccccc}
\toprule
Dataset & Method & \#Params \quad & NFE ($\downarrow$) \quad & FID ($\downarrow$) \quad & MACs ($\downarrow$) \quad & FLOPs ($\downarrow$) \\ 
\midrule 
\multirow{5}{*}{\shortstack[l]{{FFHQ}\\ {64$\times$64}}}
% & FFHQ 64$\times$64 & & & & & \\ 
% \midrule 
& EDM \cite{karras2022elucidating} (Teacher) & 55.7M & 79 & 2.47 & 82.7G & 167.9G\\
& DDIM \cite{song2020denoising}
& 55.7M & 10 & 18.30 & 82.7G & 167.9G\\
& AMED-Solver \cite{zhou2023fast} & 55.7M & 5 & 12.54 & 82.7G & 167.9G \\
& BOOT \cite{gu2023boot} & 66.9M & 1 & 9.00 & 25.3G & 52.1G \\
& \textbf{\method{}} & 27.9M & 1 & 7.21 & 26.3G & 53.8G \\
& \textbf{\method{}} & 15.7M & 1 & 7.70 & 14.8G & 30.4G \\
\midrule
 % & & & & \\ 
\midrule
\multirow{11}{*}{\shortstack[l]{{ImageNet}\\ {64$\times$64}}}
% ImageNet 64$\times$64 & & & & \\ 
& EDM \cite{karras2022elucidating} (Teacher) & 295.9M & 79 & 2.37 & 103.4G & 219.4G \\
& DDIM \cite{song2020denoising}
& 295.9M & 10 & 16.72 & 103.4G & 219.4G \\
& AMED-Solver \cite{zhou2023fast} & 295.9M & 5 & 13.75 & 103.4G & 219.4G \\
& Progressive Distillation \cite{salimans2022progressive} & 295.9M & 1 & 15.39 & 103.4G & 219.4G \\
& DSNO \cite{zheng2023fast} & 329.2M & 1 & 7.83 &  \\
& Diff-Instruct~\cite{luo2023diff}$^\dagger$ & 295.9M & 1 & 5.57 & 103.4G & 219.4G \\
& TRACT \cite{berthelot2023tract} & 295.9M & 1 & 7.43 & 103.4G & 219.4G \\
& DMD \cite{yin2024one}$^\dagger$ & 295.9M & 1 & 2.62 & 103.4G & 219.4G \\
& Consistency Model (CD) \cite{song2023consistency} & 295.9M & 1 & 6.20 & 103.4G & 219.4G \\
& Consistency Model (CT) \cite{song2023consistency} & 295.9M & 1 & 13.00 & 103.4G & 219.4G \\
& BOOT \cite{gu2023boot} & 226.5M & 1 & 16.30 & 78.2G & 157.4G \\
& \textbf{\method{}} & 80.7M & 1 & 12.34 & 31.0G & 67.8G \\
\bottomrule
\end{tabular}}
\caption{
\label{table:FFHQ_ImageNet}
Sample quality and model efficiency on FFHQ 64$\times$64 and ImageNet 64$\times$64. 
% Baseline numbers are derived from Song et al.~\cite{song2023consistency}.
$^\dagger$Methods that require adversarial-like training.
}
\end{table*}






\subsection{Discussion}
\label{sec:discussion}

\noindent\textbf{The Necessarity of 1-Flows.} Rectifying was initially designed to rectify the PF-ODE in learned flow models.
Our research indicates its effectiveness even in the absence of a base non-straight model. 
Although Annealing Rectifying does not explicitly require a pre-trained model to finetune from, acquiring valid data pairs necessitates a proficiently trained diffusion/flow model, highlighting the potential future direction of eliminating the requirement for pre-trained models.
% Moreover, in an extended experiment with randomly paired data, we could only get curved flows rather than straight flows, highlighting the potential future direction of eliminating the requirement of pre-trained models.


\noindent\textbf{Limitations.}
The performance of our approach is constrained by the capabilities of the teacher models. More precisely, it is the quality of synthetic data pairs generated by the teacher models that limit our method's performance.
% as our approach does not rely on the actual dataset on which the model was trained. 
We will investigate in the future whether the performance can be further enhanced by utilizing teacher models, real datasets, and even GAN training. 
Furthermore, we plan to adapt our method to more efficient architectures, such as transformers or pruned models.
We would also be interested in extending this work to more diffusion models such as Stable Diffusion given computation resources.

% Future investigations will explore the potential for performance enhancements by leveraging the teacher model more effectively and incorporating real data in addition to synthetic data. Furthermore, we note a more pronounced performance decline with complex datasets, which is attributable to the limitations in model capacity. 
% Moving forward, we plan to adapt our method to more efficient architectures, such as transformers, to overcome these constraints.

% The performance of our method is limited by the teacher model. To be specific, the performance of the method is limited by the synthetic data pairs generated by the teacher model as we do not need the true data set the model is trained on. 
% Additionally, we observe a larger drop on more sophisticated datasets and this is related to model capacity.
% We intend to apply our method to other more efficient architectures like transformers in the future.

==> text/method_old.tex <==
% \section{Toward Smaller One-Step Models}
\section{\method{}}
\label{sec:method}

% In \cref{sec:general_flow}, we start by discussing some drawbacks when applying the ReFlow pipeline to smaller models directly and show that Rectifying is a general method for straightening the empirical PF-ODE of diffusion models.
% In \cref{sec:an_flow}, we introduce the Annealing Rectifying technique along with special data augmentation to get smaller 2-flow models.
% Then, we describe a new loss to help distill a compact one-step model with extra regulation from 2-flow models in \cref{sec:distill}
In this section, we introduce the \method{} framework for learning small one-step generative models.
To effectively exploit the Rectified Flow framework in our setting, \method{} improves both reflow and distillation.
The first part, Annealing Reflow, provides a new technique for the initialization of reflow. It smoothly transforms from training a 1-rectified flow to training a 2-rectified flow, giving the small student model a warm-start initialization and accelerate the training convergence.
The second part, Flow-Guided Distillation

\subsection{Annealing Reflow}

\iffalse
% \subsection{Initialization of Small Model: annealing Rectifying}
\subsection{Annealing Rectifying}
\label{sec:an_flow}
% \noindent\textbf{General Straightening Strategy.} 

\noindent\textbf{Annealing Rectifying.}
The Rectifying mentioned in \cref{sec:reflow} needs to first train a 1-flow and then use it to generate data pairs for Rectifying.
In the Rectifying procedure, we can initialize from the previous flow when the model size is the same, But we can not do it when the architecture is different.
In this section, we introduce Annealing Rectifying to overcome these issues.
Recent advancements have unveiled that the coupling learned by neural networks in diffusion and flow-based generative models is both stable and robust, as highlighted in recent studies \cite{zhang2023emergence, khrulkov2022understanding, kadkhodaie2023generalization}. This finding indicates that given the same initial noise, the final samples produced by the PF-ODE across various diffusion schedules remain unchanged.
For any diffusion process $x_t = \alpha_t x_1 + \sigma_t x_0$ with schedule $\{\alpha_t, \sigma_t\}$, where $\alpha_1 = 1$, $\sigma_1=0$, $\alpha_0/\sigma_0 = 0$ and the log Signal-to-Noise Ratio (SNR) $\lambda_t=\log[(\alpha_t / \sigma_t)^2]$ increases monotonically with $t$,
the general PF-ODE can be rewritten as:
\begin{equation}\label{eq:pf_ode_lambda}
\mathrm{d}\left(\frac{\mathbf{x}_\lambda}{\alpha_\lambda}\right) = \frac{1}{2} \left( D(\mathbf{x}_\lambda, \lambda) - \frac{\mathbf{x}_\lambda}{\alpha_\lambda} \right)\mathrm{d}\lambda
\end{equation}
where $D$ is the denoiser, which always predicts the clean image based on the noisy input $\mathbf{x}_\lambda$ and satisfy $\nabla_\mathbf{x} \log p_t(\mathbf{x}) = \frac{\alpha_t D(x_t,t) - x_t}{\sigma_t^2}$.
In some recent works, researchers show the equivariance between different representations such as score and velocity \cite{salimans2022progressive, kingma2024understanding}. That is to say, for diffusion and flow-based models with different schedule $\{\alpha_t, \sigma_t\}$, as long as the neural networks are fitted well, according to \cref{eq:pf_ode_lambda}, the generated samples for the same initial point will be similar.
% In some works \cite{yin2023one, xing2023exploring}, researchers used the same hypothesis to utilize generated data from other diffusion models.
In this work, we will use data pairs generated by the other diffusion models such as EDM for Annealing Rectifying.

Given data pairs $(\mathbf{z}_0,\mathbf{z}_1)$ from a big teacher model, we can combine the training of 1-flow models with the Rectifying in an annealing manner. Unlike in the Rectifying where $\mathbf{z}_t = t \mathbf{z}_1 + (1-t) \mathbf{z}_0$, we introduce adaptive randomness to the interpolation of the pairs:
\begin{equation}\label{eq:scale_pair}
    \mathbf{z}_t^{\beta} = t \mathbf{z}_1 + (1-t) \left(\sqrt{1-\beta^2(\text{step})} \mathbf{z}_0 + \beta(\text{step}) \mathbf{\epsilon}\right) =  t \mathbf{z}_1 + (1-t) \mathbf{z}_0^{\beta},
\end{equation}
where $\beta \in [0,1]$ is a scaler changing with training steps, $\mathbf{\epsilon}$ is a random \textit{independent} sample from initial distribution $\pi_0$, $\mathbf{z}^{\beta}_0$ is the approximated spherical linear interpolation between $\mathbf{z}_0$ and $\epsilon$.
When $\beta$ is set to 1, the training aligns with flow matching. On the other hand, setting $\beta=0$ corresponds to the original Rectifying.
The training objective of Annealing Rectifying is a modified version of \cref{eq:objective_reflow}:
\begin{equation}\label{eq:objective_an_reflow}
\begin{aligned}
   \mathbb{E}_{t}\Big\{\gamma(t) \mathbb{E}_{(\mathbf{z}_0, \mathbf{z}_1, \epsilon)}
   \big[\|\mathbf{v}_\theta(t\mathbf{z}_1+(1-t)\mathbf{z}^{\beta}_0, t) - (\mathbf{z}_1 - \mathbf{z}^{\beta}_0) \|_2^2 \big]\Big\},
\end{aligned}
\end{equation}
where $\mathbf{z}^{\beta}_0 = \sqrt{1-\beta^2(\text{step})} \mathbf{z}_0 + \beta(\text{step}) \mathbf{\epsilon}$. The training pipeline is illustrated in \cref{fig:main_a} and we denote the resulting model as $\mathbf{v}_{\text{2-flow}}$.

% \begin{algorithm}[!b]
%     \small
%    \caption{Annealing ReFlow Algorithm}
%    \label{alg:annealing_reflow}
%     \begin{algorithmic}[1]
%      \Require paired dataset $\mathcal{D}$, randomness schedule $\beta$, learn rate $\eta$, $d(\cdot,\cdot)$, $w(t)$
%     % \State{Initialize $\mathbf{v}_{\theta}$ with $\mathbf{v}_{\text{2-flow}}$}
%         \Repeat
%         \State{Sample $\mathbf{z}_0, \mathbf{z}_1 \sim \mathcal{D}$}
%         \State{Sample $\epsilon \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$ and $t \sim \mathcal{U}(\epsilon,1)$}
%         \State{calculate $\mathbf{z}^\beta_0 = \sqrt{1-\beta(\text{step})^2} \mathbf{z}_0 + \beta(\text{step}) \mathbf{\epsilon}$ and $\mathbf{z}^\beta_t = t \mathbf{z}_1 + (1-t) \mathbf{z}^\beta_0$}
%         \State{$\mathcal{L}_{\text{AnReFlow}}(\theta) \leftarrow w(t) d(\mathbf{v}_\theta(\mathbf{z}^\beta_t,t), \mathbf{z}_1 - \mathbf{z}^\beta_0)$}
%         \State{$\theta \leftarrow \theta - \eta \nabla_\theta \mathcal{L}_{\text{AnReFlow}}(\theta)$}
%         \Until{convergence}
%     \end{algorithmic}
% \end{algorithm}

\begin{figure}[!t]
\centering
\begin{overpic}[width=1.\linewidth]{figures/symmetry}% no need to specify the file extension
% \put(76.5, 1.){\color{gray}{\line(0,1){41.4}}}
\put(1.5,32){\color{black}{(a)}}
\put(39.5,32){\color{black}{(b)}}
\put(78,32){\color{black}{(c)}}
\end{overpic}
\caption{(a) Samples generated with the model trained without any data augmentation. (b) Samples generated with a model trained with horizontal flip using the same initial noise. (c) Three image pairs generated with the model trained without any data augmentation using PF-ODE. From top to bottom: random noise and sample generated, horizontally flipped noise and corresponding sample, vertically flipped noise and corresponding sample.
% \textcolor{red}{quantitatively compute (c)}
}
\label{fig:symmetry}
\end{figure}

Since $\mathbf{z}_0$ is from $\pi_0$ and $\pi_0$ is the standard Gaussian distribution, we have $\mathrm{Law}(\mathbf{z}_0^{\beta})=\pi_0$. 
Additionally, the marginal preserving property of rectified flows also holds for $\mathbf{z}_t^{\beta}$ no matter the value of $\beta$, which reads $\mathrm{Law}(\mathbf{z}_t^{\beta})=\mathrm{Law}(\mathbf{z}_t)$. 
% In Appendix \ref{append:beta_flow}, we present the one-step and multi-step results of models trained with different fixed $\beta$ values.
In the Appendix, we present the one-step and multi-step results of models trained with different fixed $\beta$ values.
\cref{eq:scale_pair} provides a connection between the flow matching and Rectifying and points out that the key difference lies in the randomness of the data pairs. 
% For more discussion on this, see Appendix \ref{append:comparison_fm}.




\noindent\textbf{Intrinsic Symmetry of Nature Images.}
While the coupling is robust no matter what kind of diffusion we use, we discover that there exists an intrinsic symmetry of diffusion (see \cref{fig:symmetry}).
% we first notice that two diffusion models trained on the same dataset, one with horizontal flip data augmentation and another without. for the same input noise, the data samples generated according to the PF-ODE are almost the same. 
We initially observed that when two diffusion models are trained on an identical dataset—with one model utilizing horizontal flip data augmentation and the other not—the data samples generated from the same input noise are remarkably similar according to the PF-ODE.
Furthermore, we show that for a model trained without any data augmentation, applying a horizontal flip to the initial noise results in a horizontally flipped generated image.
This implies a data augmentation on the data pairs for the Rectifying that could potentially decrease the number of simulations of the teacher models.
% We further calculate the MSE loss between images generated with a batch of initial noise and with noise under certain operations.
\fi

\iffalse
\subsection{Distillation with Guidance from 2-Flow}
\label{sec:distill}
% We note that to get a distilled one-step model in our framework, there are three factors we should take into consideration. (i) the data pairs used for training, (ii) the initialization of the student model, (iii) The training algorithm to use

% Previously, in Rectified Flows, the distillation was done with data pairs generated from 2-flows, initialization from 2flow and naive training objective:
In the distillation stage, we want to distill the 2-flows $\mathbf{v}_{\text{2-flow}}$ trained with Annealing Rectifying into one-step models $\mathbf{v}_{\phi}$.
Previously, in Rectified Flows, the distillation was done with data pairs generated from 2-flows and the training objective is straightforward:
\begin{equation}\label{eq:simple_dis}
    \mathcal{L}_{\text{dis}} = \mathbb{E}_{(\mathbf{z}_0,\mathbf{z}_1)} \left[d( \mathbf{v}_\phi(\mathbf{z}_0,0), (\mathbf{z}_1-\mathbf{z}_0))\right],
\end{equation}
where $(\mathbf{z}_0,\mathbf{z}_1)$ are data pairs generated with 2-flows, $d$ can be MSE loss or perceptual loss such as Learned Perceptual Image Patch Similarity (LPIPS) loss.
We noticed that the performance of distilled flows is in general worse than that of corresponding (few-steps) 2-flows in \cite{liu2022rectified}.
The straighter trajectories and fewer step generation characteristics of 2-flows have led us to utilize 2-flows in the distillation stage as an additional source of supervision. 
% Based on the observation that 2-flows are straight and support few steps generation, we proposed to bring 2-flows as teacher models to help the distillation process.

% date generation is time-consuming and we want to avoid it by utilizing the information in the 2-flow models. 
The new loss term is inspired by Heun's method used in EDM \cite{karras2022elucidating}.
% Inspired by Heun's method used in EDM \cite{karras2022elucidating} and by showing the straightness of the 2 flow model, we propose a new loss:
% \begin{equation}\label{eq:new_dis}
%     L_{\text{teacher}} = \mathbb{E}_{X_0\sim\mathcal{N}, t\sim\mathcal{U}} d( sg[v_{\text{teacher}}(X_0 + t * v_\theta(X_0), t)], v_\theta(X_0) ),
% \end{equation}
% where sg stands for stop gradient. For more details, please refer to Appendix \ref{append:teacher_loss} 
For initial value problems of the form:
\begin{equation}\label{eq:init_ode}
  \mathrm{d}\mathbf{x}(t) = f(\mathbf{x}(t),t)\mathrm{d}t, 
\end{equation}
Heun's method, an improved Euler's method, first calculates the intermediate value $\Tilde{x}_{i+1}$ and then the final approximation $x_{i+1}$ based on the current state $x_i$:
\begin{equation}\label{eq:heun_ori}
  \begin{aligned}
  {\tilde {\mathbf{x}}}_{i+1}&=\mathbf{x}_{i}+hf(\mathbf{x}_{i},t_{i})  \\ 
  { {\mathbf{x}}}_{i+1}&=\mathbf{x}_{i}+\frac{h}{2}\left[f(\mathbf{x}_{i},t_{i}) + f({\tilde {\mathbf{x}}}_{i+1} ,t_{i+1})\right] 
  \end{aligned}
\end{equation}
where $h= t_{i+1} - t_i$ is the step size.
To train a distilled model $\mathbf{v}_\phi$, we would assume the current time step is always $t_i=0$. Also since $t_{i+1}$ is not recognized by $\mathbf{v}_\phi$, we would replace the function for the second evaluation with the 2-flow model $\mathbf{v}_{\text{2-flow}}$. As a result, we have:
\begin{equation}\label{eq:heun_new}
  \begin{aligned}
  {\tilde {\mathbf{z}}}_{t} &= \mathbf{z}_{0}+t \mathbf{v}_\phi(\mathbf{z}_{0}, 0)  \\ 
  {\mathbf{z}}_{t} &= \mathbf{z}_{0}+\frac{t}{2}\left[\mathbf{v}_\phi(\mathbf{z}_{0}, 0) + \mathbf{v}_{\text{2-flow}}({\tilde {\mathbf{z}}}_{t}, t)\right] 
  \end{aligned}
\end{equation}
% where we adapt the notations in the main text for consistency.

Assume ${\mathbf{z}}_{t}$ is a better estimation than ${\tilde {\mathbf{z}}}_{t}$, we get immediately a new objective:
\begin{equation}\label{eq:new_dis_appen}
  \begin{aligned}
    \mathcal{L}_{\text{2-flow}} &=  \mathbb{E}_{\mathbf{z}_0; t} \left[d\left({\mathbf{z}}_{t}, {\tilde {\mathbf{z}}}_{t}\right)\right] \\ &= \mathbb{E}_{\mathbf{z}_0; t} \big[w(t) d\left( \text{sg}[\mathbf{v}_{\text{2-flow}}(\mathbf{z}_0 + t * \mathbf{v}_\phi(\mathbf{z}_0, 0), t)], \mathbf{v}_\phi(\mathbf{z}_0, 0) \right)\big],
  \end{aligned}
\end{equation}
where $\mathbf{z}_0\sim \pi_0$ can be outside of paired dataset $\mathcal{D}$, $t$ is uniformly sampled over the continuous interval $[0, 1]$, sg stands for stop gradient, $w(t)$ is the weight of the loss, and we have $w(t) = t^2/4$ when $d(\cdot, \cdot)$ is the $l_2$ distance. In practice, we use the LPIPS distance and set $w(t) = 1$. We summarize the distillation algorithm in \cref{alg:Distillation}.

\begin{algorithm}[H]
    \small
   \caption{Distillation Algorithm}
   \label{alg:Distillation}
    \begin{algorithmic}[1]
     \Require paired dataset $\mathcal{D}$, $\mathbf{v}_{\text{2-flow}}$, learn rate $\eta$, $d(\cdot,\cdot)$, $w(t)$
    \State{Initialize $\mathbf{v}_{\phi}$ with $\mathbf{v}_{\text{2-flow}}$}
        \Repeat
        \State{Sample $\mathbf{z}_0, \mathbf{z}_1 \sim \mathcal{D}$}
        \State{$\mathcal{L}_{\text{dis}}(\phi) \leftarrow d(\mathbf{v}_{\phi}(\mathbf{z}_0,0),\mathbf{z}_1-\mathbf{z}_0)$}
        \State{Sample $\mathbf{z}'_0 \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$ and $t \sim \mathcal{U}(\epsilon,1)$} \textcolor[rgb]{0.40,0.40,0.40}{{\textit{// data outside paired dataset $\mathcal{D}$}}}
        \State{Inference with $\mathbf{z}'_0$ using student model $\rightarrow \mathbf{v}_\phi(\mathbf{z}'_0,0)$ }
        \State{Calculate intermediate state $\mathbf{z}'_t = \mathbf{z}'_0 + t * \mathbf{v}_\phi(\mathbf{z}'_0,0)$}
        \State{$\mathcal{L}_{\text{2-flow}}(\phi) \leftarrow w(t) d(\mathbf{v}_\phi(\mathbf{z}'_0,0), \text{sg}[\mathbf{v}_{\text{2-flow}}(\mathbf{z}'_t, t)])$}
        \State{$\phi \leftarrow \phi - \eta \nabla_\phi (\mathcal{L}_{\text{dis}}(\phi) + \mathcal{L}_{\text{2-flow}}(\phi))$}
        \Until{convergence}
    \end{algorithmic}
\end{algorithm}
\fi

==> text/related_old.tex <==
\section{Related Work}
\xc{TODO: polish}

\noindent\textbf{Fast ODE Solver.}
With the new perspective of viewing the diffusion sampling process as solving the corresponding PF-ODE \cite{song2020score}, numerous methods are introduced to accelerate the diffusion sampling process with minimum loss of generation quality.
Some of the representative work in this area are DDIM \cite{song2020denoising}, EDM \cite{karras2022elucidating}, DEIS \cite{zhang2022fast} and DPM-solver \cite{lu2022dpm}.
Based on the property of the diffusion sampling trajectory, Zhou \etal introduced AMED-Solver which utilizes the mean value theorem to minimize the discretization error and requires even fewer NFE for image generation \cite{zhou2023fast}.

\noindent\textbf{Diffusion Distillation.}
% \noindent\textbf{Diffusion Trajectory Distillation}
Beyond these fast ODE salvers, distillation-based methods aim to achieve one-step sampling. 
The success of diffusion distillation fundamentally relies on leveraging the learned empirical PF-ODE trajectory.
% The key to the success of diffusion distillation is to utilize the information from the learned empirical PF-ODE trajectory. 
Salimans \etal \cite{salimans2022progressive} proposed to repeatedly train a student network whose stepsize is twice the teacher's and set the student as a new teacher for the next round.
Gu \etal \cite{gu2023boot} suggested distilling the knowledge of the teacher models in a data-free manner with the help of the signal-ODE.
Yin \etal \cite{yin2024one} extended the idea of variational score distillation from previous work in 3D \cite{wang2023prolificdreamer} to train a one-step generator by alternatively updating the one-step generator and a fake data score function.
% which achieves the state-of-the-art performance on both SD and toy datasets like cifar10.
Additionally, adversarial training is introduced in many methods to help train a one-step model or improve the performance of one-step diffusion models \cite{ye2023score,kim2023consistency,xu2023ufogen}.

\noindent\textbf{Consistency Models \cite{song2023consistency}.}
Recently, Song \etal proposed consistency models as a new family of generative models.
These models imposed consistency constraints on the predictions of models at two consecutive data points on the same trajectory:
\begin{equation}\label{eq:cm_loss}
    \mathcal{L}_{\text{cm}} = \mathbb{E}_{t}\Big\{\gamma(t) \mathbb{E}_{\mathbf{x}_t \sim q(\mathbf{x}_t|\mathbf{x})} d(D_\theta(\mathbf{x}_t, t), D_{\theta^-}(\mathbf{x}_s, s) )\Big\},
\end{equation}
where $\gamma(t)$ is a positive weight coefficient, $\mathbf{x} \sim p_{\mathrm{data}}$, $\theta^-$ represents the Exponential Moving Average (EMA) of the parameters $\theta$ of the consistency models, $D$ is the consistency function which self-consistent property. 
$\mathbf{x}_s$ is a closer state to $\mathbf{x}$ than $\mathbf{x}_t$.
Consistency models utilize two training methods:  Consistency Distillation (CD) and Consistency Training (CT).
In CD, $\mathbf{x}_s$ is obtained by a one-step update of the ODE-solver applied to the empirical PF-ODE.
In CT, $\mathbf{x}_s\sim q(\mathbf{x}_s|\mathbf{x})$ is sampled in a manner akin to $\mathbf{x}_t$.
% is obtained by adding noise according to the forward diffusion process.
% In \cite{song2023improved}, Song \etal presented improved techniques for consistency training and achieved much lower FID in image generation.
